Body Transformer: Leveraging Robot Embodiment for Policy Learning

In recent years, the transformer architecture has become the de facto standard for machine learning algorithms applied to natural language processing and computer vision. Despite notable evidence of successful deployment of this architecture in the context of robot learning, we claim that vanilla transformers do not fully exploit the structure of the robot learning problem. Therefore, we propose Body Transformer (BoT), an architecture that leverages the robot embodiment by providing an inductive bias that guides the learning process. We represent the robot body as a graph of sensors and actuators, and rely on masked attention to pool information throughout the architecture. The resulting architecture outperforms the vanilla transformer, as well as the classical multilayer perceptron, in terms of task completion, scaling properties, and computational efficiency when representing either imitation or reinforcement learning policies. Additional material including the open-source code is available at https://sferrazza.cc/bot_site.

==> tex/runtime-performance-rearranged.tex <==
\begin{figure*}[ht]
    \centering
    \begin{subfigure}[t]{\textwidth}
        \centering
        \includegraphics[width=0.3\textwidth]{figures/computational_runtime_way_smaller.pdf}
        \hspace{0.05\textwidth}
        \includegraphics[width=0.5\textwidth]{figures/computational_flop_way_smaller.pdf}
        \caption{
            \textbf{Computational Analysis for Increasing Number of Nodes.}
            Across 10,000 randomly sampled masks, we found that our custom implementation provides a $200\%$ speed-up in runtime (shown at left) at sequence lengths up to 128 nodes and scales better in number of FLOPs (shown at right). The mask is assumed as sparse as the one used for MoCapAct experiments.
        }
        \label{fig:runtime-and-flops}
    \end{subfigure}
    % \begin{subfigure}[t]{\textwidth}
    %     \centering
    %     \includegraphics[width=0.3\textwidth]{figures/computational_runtime_16.pdf}
    %     \hspace{0.03\textwidth}
    %     \includegraphics[width=0.3\textwidth]{figures/computational_runtime_32.pdf}
    %     \hspace{0.03\textwidth}
    %     \includegraphics[width=0.3\textwidth]{figures/computational_runtime_64.pdf}
    %     \caption{
    %         \hl{\textbf{Computational analysis w.r.t. Sparsity.}
    %         Across 50,000 randomly sampled masks for each mask size $16 \times 16$ (left), $32 \times 32$ (center), and $64 \times 64$ (right), runtime scales inversely linearly with mask sparsity, and is more efficient until a mask density of $0.4$-- higher than any mask we adopted in this paper.}
    %     }
    %     \label{fig:sparsity}
    % \end{subfigure}
    \caption{
    \textbf{Computational analysis of the custom masked attention implementation.}
    }
    \label{fig:computational-analysis}
    \vspace{-5mm}
\end{figure*}
